Is Gender "In-the-Wild" Inference Really a Solved Problem?

Soft biometrics analysis is seen as an important research topic, given its relevance to various applications. However, even though it is frequently seen as a solved task, it can still be very hard to perform in wild conditions, under varying image conditions, uncooperative poses, and occlusions. Considering the gender trait as our topic of study, we report an extensive analysis of the feasibility of its inference regarding image (resolution, luminosity, and blurriness) and subject-based features (face and body keypoints confidence). Using three state-of-the-art datasets (PETA, PA-100K, RAP) and five Person Attribute Recognition models, we correlate feature analysis with gender inference accuracy using the Shapley value, enabling us to perceive the importance of each image/subject-based feature. Furthermore, we analyze face-based gender inference and assess the pose effect on it. Our results suggest that: 1) image-based features are more influential for low-quality data; 2) an increase in image quality translates into higher subject-based feature importance; 3) face-based gender inference accuracy correlates with image quality increase; and 4) subjects' frontal pose promotes an implicit attention towards the face. The reported results are seen as a basis for subsequent developments of inference approaches in uncontrolled outdoor environments, which typically correspond to visual surveillance conditions.

==> article/exp_backup.tex <==

\section{Experiments}

\subsection{Dataset and Evaluation Metrics}
% General description. Try to reuse common article information. Split between face and pedestrian datasets, as well as its evaluation metrics (face dataset, Adience, has only \%)

% \subsection{Implementation Details}
% Description of method implementations and variations of said implementations (APR and other). Details of implementation for the face gender method (based on StrongBaseline with transform and loss function difference). Gender evaluation of methods was done by only calculation loss for that specific attribute.

We conduct experiments for gender prediction in wild conditions using three pedestrian attribute datasets: PETA \cite{deng2014pedestrian}, RAP \cite{li2016richly} , and PA100k \cite{liu2017hydraplus}. The PETA dataset consists of 19000 images with 61 binary attributes. It is divided into three subsets: 9500 for training, 1900 for validation and 7600 for testing. Following the established protocol for this dataset, we report the results on the 35 attributes with a ratio of positive labels higher than 5\%. The RAP dataset contains 41585 images, each annotated with 72 attributes. Following the official protocol \cite{li2016richly}, we split the dataset into 33,268 training images and 8,317 test images and reported results on the 51 binary attributes with a positive ratio higher than 1\%. The PA-100K dataset is composed of 100000 images from outdoor surveillance cameras. It is split into 80000 images for training, 10000 for validation and 10000 for testing. Each image is annotated with 26 attributes.

To display our results of selected methods on each dataset, we used two types of metrics [16]: label-based and instance-based metrics. For the label-based metric, we computed the mean Accuracy (mA), which is the mean value of classification accuracy of positive and negative samples for each attribute, averaging over all attributes.  The mA criterion can be formulated as:

\begin{equation}
mA = \dfrac{1}{2N} \sum_{i=1}^{M} \left(\dfrac{TP_i}{P_i} + \dfrac{TN_i}{N_i} \right)
\end{equation}

where \textit{N} is the number of examples, \textit{M} the number of attributes. 
\textit{$TP_i$}  is the number of positive examples and \textit{$TP_i$} the number of correctly predicted positive examples for the $i^{th}$ attribute; \textit{$TN_i$} and \textit{$N_i$} are defined analogously. For instance-based metrics, we used accuracy, recall, precision and F1 score.

% TODO: 
% Como calcular o género
% Justificar escolhas de métodos e de datasets

\subsection{Implementation Details}
% Description of method implementations and variations of said implementations (APR and other). Details of implementation for the face gender method (based on StrongBaseline with transform and loss function difference). Gender evaluation of methods was done by only calculation loss for that specific attribute.
\subsubsection{Methods Adaptations}

The models used were VAC \cite{guo2019visual}, ARP \cite{lin2019improving}, ALM \cite{tang2019improving}, StrongBase \cite{jia2020rethinking}, and DeepMar \cite{li2015multi}. We used the authors' implementation as closely as possible in our experiments. However, we had to modify some implementation details to make a fair comparison between models and to combine models' gender predictions in our experiments. 

VAC model test and train transformation for PETA and RAP were based on their WIDER  dataset \cite{li2016human} transformation. Additionally, attribute weights for weighted sigmoid cross-entropy loss \cite{li2015multi} calculation were only defined for PA-100K. We retrieve attribute weights for PETA and RAP from the same source the authors used to obtain the PA-100K ones. We raised the number of training epochs to 30 to keep it consistent across other model implementations. Additionally, to allow gender prediction comparison for our experiments, we changed the PETA dataset evaluation for the StrongBase's evaluation implementation. Gender evaluation was done by adjusting the output-related loss without modifying attention-related losses.

For ARP, we only considered attribute loss, ignoring the re-identification one. The available implementation did not consider PETA, RAP, and PA-100K dataset evaluation, so we introduced it following the paper guidelines. For PETA, the model was trained for 60 epochs, reducing its learning rate to 0.001 in the last 20 epochs. The approach was similar for RAP and PA-100K, with training lasting 30 epochs and the learning rate reduction occurring in the last ten epochs.

The remaining models were evaluated using their available implementation. For all models' implementations that did not consider the evaluated datasets, we incorporated StrongBase dataset reading into their implementation. For consistency purposes, all metric evaluation was also based on StrongBase implementation.

\subsubsection{Face Gender Model}

The proposed method is based on StrongBase implementation \cite{jia2020rethinking}, using PyTorch and trained end-to-end.  ResNet50 \cite{he2016deep} is adopted as backbone to extract pedestrian image features. The model is separated into feature exactor and classifier parts. The feature extractor is ResNet50 without its average pool and fully connected layer, which were incorporated in the classifier part. The fully connected layer was replaced by a linear layer followed by a batch normalization layer.  Pedestrian images are resized to $256\times192$ with random horizontal mirroring as inputs. Stochastic Gradient Descent (SGD) is employed for training, with momentum of $0.9$, and weight decay of $0.0005$.  The initial learning rate is $0.01$ for the feature extractor and $0.1$ for the classifier part. Plateau learning rate scheduler is used with a reduction factor of $0.1$ and a patience epoch number of $4$. Batch size is set to $64$ and the total epoch number of training is $30$.

\subsection{Cross Domain Performance}

% Values of all selected methods for datasets. Refer that some do not have reported values and VAC has lower score given that we used StrongBaseline metric calculation and PETA split (which differed from the one used in VAC) for method comparison integrity.
% Include here cross evaluation done. Refer that from its analysis, training gender specifically or not has little impact and that models trainde from RAP appear to faulter in other dataset performance. Since this is the case, we intent to explore what features each dataset has that might contribute to gender prediction.

We first train the selected models in the considered datasets to validate gender prediction analysis. We present the obtained results in Table \ref{table:reported_results}. The metric values exhibited refer to all attributes of each dataset and not only gender. There are some models which were not evaluated, in their papers, for all of the datasets we considered. As such, we can not compare our results and the reported ones in these cases. However, when comparing reported results to our own, we observe that their results are similar to those we report. Thus, we can conclude that our model manipulation and training do not influence our experiments' reported gender prediction results. The more discrepant case is VAC evaluated in PETA, where we report lower metric values than those of the original paper. Nevertheless, this situation can be explained by the PETA evaluation change we induced in this model to enable comparison between methods' gender prediction in our experiments.

% \begin{table*}[!htb]
%     \renewcommand{\arraystretch}{1.2}
%     \caption{Pedestrian attribute metric values in PETA dataset.}
%     \begin{tabular}{c*{5}c|*{5}c|*{5}c}\\\hline
%         \multirow{2}{*}{\textbf{Methods}} & \multicolumn{5}{c|}{PETA}
%         & \multicolumn{5}{c|}{RAP} & \multicolumn{5}{c}{PA-100K} \\

%         &\makebox[1em]{\footnotesize mA}
%         &\makebox[1em]{\footnotesize Acc}
%         &\makebox[1em]{\footnotesize Prec}&\makebox[1em]{\footnotesize Recall}&\makebox[1em]{\footnotesize F1}
        
%         &\makebox[1em]{\footnotesize mA}
%         &\makebox[1em]{\footnotesize Acc}
%         &\makebox[1em]{\footnotesize Prec}&\makebox[1em]{\footnotesize Recall}&\makebox[1em]{\footnotesize F1}
        
%         &\makebox[1em]{\footnotesize mA}
%         &\makebox[1em]{\footnotesize Acc}
%         &\makebox[1em]{\footnotesize Prec}&\makebox[1em]{\footnotesize Recall}&\makebox[1em]{\footnotesize F1}
%         % &\makebox[4em]{\footnotesize Gender Acc}
%         \\\hline\hline

%         VAC \cite{guo2019visual} &
%         % mA 
%         82.34 & 
%         % Acc, Prec, Recall, F1
%         78.80 & \textbf{89.15} & 84.08 & 86.16 &
        
%         % mA 
%         75.11 & 
%         % Acc, Prec, Recall, F1
%         68.34 & \textbf{83.52} & 77.25 & 79.84 &
        
%         78.20 & 
%         % Acc, Prec, Recall, F1
%         \textbf{79.80} & \textbf{90.95} & 84.98 & \textbf{87.44} \\
        
%         % Modelo
%         ALM \cite{tang2019improving} &
%         % mA 
%         82.48 & 
%         % Acc, Prec, Recall, F1
%         77.25 & 85.24 & 85.61 & 85.13 & 
        
%          % mA 
%         \textbf{80.68} & 
%         % Acc, Prec, Recall, F1
%         66.73 & 73.69 & \textbf{86.19} & 78.99 &
        
%         % mA 
%         78.75 & 
%         % Acc, Prec, Recall, F1
%         75.80 & 82.94 & \textbf{87.78} & 84.79 \\
        
%         % Modelo
%         APR \cite{lin2019improving} &
%         % mA 
%         82.83 & 
%         % Acc, Prec, Recall, F1
%         77.90 & 86.99 & 84.69 & 85.52 &
        
%         % mA 
%         73.44 & 
%         % Acc, Prec, Recall, F1
%         67.12 & 82.39 & 76.33 & 78.85 &
        
%         % mA 
%         77.33 & 
%         % Acc, Prec, Recall, F1
%         78.00 & 88.34 & 85.08 & 86.24\\
        
%         % Modelo
%         DeepMar \cite{li2015multi} &
%         % mA 
%         83.89 & 
%         % Acc, Prec, Recall, F1
%         76.81 & 85.16 & 84.81 & 84.98 &
        
%         % mA 
%         77.06 & 
%         % Acc, Prec, Recall, F1
%         64.05 & 76.46 & 77.96 & 76.70 & 
        
%         % mA 
%         79.26 & 
%         % Acc, Prec, Recall, F1
%         76.48 & 85.49 & 85.71 & 85.15 \\

%         % Modelo
%         StrongBase \cite{jia2020rethinking} &
%         % mA 
%         \textbf{85.30} & 
%         % Acc, Prec, Recall, F1
%         \textbf{79.00} & 86.62 & \textbf{86.52} & \textbf{86.30} &
        
%         % mA 
%         80.61 & 
%         % Acc, Prec, Recall, F1
%         \textbf{68.63} & 79.86 & 81.13 & \textbf{80.10} & 
        
%         % mA 
%         \textbf{80.55} & 
%         % Acc, Prec, Recall, F1
%         79.06 & 87.51 & 87.13 & 86.93 \\
    

%         \hline
%     \label{table:reported_results}
%     \end{tabular}
% \end{table*}


In our first experiment, we evaluate gender prediction for each model in each dataset. Furthermore, we intend to examine each model's performance in datasets for which they were not trained. This analysis highlights potential differences between models and datasets regarding gender prediction. Additionally, we train each model specifically for the gender attribute and compare its performance with a corresponding model trained for all dataset attributes. We report our results in Table \ref{table:cross_domain}.



\begin{table}[!t]
    \centering
    \renewcommand{\arraystretch}{1.1}
    \caption{Gender accuracy, expressed by mA metric of different dataset trained models on various pedestrian attribute datasets. Models with Gender termination refer to models trained solely for gender attribute.}
    \begin{tabular}{|c||*{4}{c|}}\hline
        \backslashbox{\textbf{Train}}{\textbf{Eval}} & \textbf{Methods} & \multicolumn{1}{c|}{\textbf{PETA}}  & \multicolumn{1}{c|}{\textbf{RAP}} & \multicolumn{1}{c|}{\textbf{PA-100K}} \\\hline
        
        \multirow{10}{*}{PETA} &
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%% PETA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Modelo
        StrongBase &
        % PETA 
        92.80 & 
        % RAP
        79.47 &
        % PA-100K 
        78.98 \\

        % Modelo
         &
        StrongBase-Gender &
        % PETA 
        \textbf{93.13} & 
        % RAP 
        80.44 & 
        % PA-100K
        79.65 \\
        
        \cline{2-5}
        
        &
        % Modelo
        ALM &
        91.36 & 
        % RAP
        80.62 &
        % PA-100K
        76.95 \\
        
        % Modelo
         &
        ALM-Gender & 
        % PETA 
        92.28 & 
        % RAP
        82.66 &
        % PA-100K
        78.27 \\
        
        \cline{2-5}
        
        % Modelo
        &
        DeepMar &
        % PETA 
        91.08 & 
        % RAP
        71.76 & 
        % PA-100K
        72.83 \\
        
         % Modelo
        &
        DeepMar-Gender &
        % PETA 
        92.33 & 
        % RAP
        74.78 &
        % PA-100K
        77.63 \\
        
        \cline{2-5}
        
        % Modelo
        &
        VAC &
        % PETA 
        92.85 & 
        % RAP
        78.50 & 
        % PA-100K
        78.16 \\
        
        % Modelo
        &
        VAC-Gender &
        % PETA 
        92.76 & 
        % RAP
        77.92 & 
        % PA-100K
        78.22 \\
        
        
        \cline{2-5}
        
        
        % Modelo
        &
        APR &
        % PETA 
        92.84 & 
        % RAP
        78.95 & 
        % PA-100K
        78.83 \\
        
        % Modelo
        &
        APR-Gender &
        % PETA 
        92.34 & 
        % RAP
        78.49 &
        % PA-100K
        75.49 \\
        
        \hline
        \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%% RAP %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \multirow{10}{*}{RAP} &
        StrongBase &
        % PETA 
        63.75 &
        % RAP
        96.94 & 
        % PA-100K
        73.19  \\
        
        &
        StrongBase-Gender &
        % PETA 
        71.41 &
        % RAP
        96.34 & 
        % PA-100K
        76.97 \\ 
        
        
        \cline{2-5}
        
        &
        % Modelo
        ALM &
        % PETA 
        76.81 &
        % RAP
        95.69 & 
        % PA-100K
        81.24 \\
        
        &
        ALM-Gender &
        % PETA 
        76.03 &
        % RAP
        95.41 & 
        % PA-100K
        80.28 \\ 

        \cline{2-5}
        % Modelo
        &
        DeepMar &
        % PETA 
        69.29 &
        % RAP
        95.52 & 
        % PA-100K
        75.76 \\

         % Modelo
        &
        DeepMar-Gender &
        % PETA 
        70.22 &
        % RAP
        96.40 & 
        % PA-100K
        76.89 \\
        
        \cline{2-5}
        
        % Modelo
        &
        VAC &
        % PETA 
        71.27 &
        % RAP
        \textbf{97.04} & 
        % PA-100K
        73.72 \\

        % Modelo
        &
        VAC-Gender &
        % PETA 
        72.89 &
        % RAP
        96.59 & 
        % PA-100K
        76.67 \\
        
        \cline{2-5}
        % Modelo
        &
        APR &
        % PETA 
        68.39 &
        % RAP
        96.20 & 
        % PA-100K
        75.41 \\
        
        % Modelo
        &
        APR-Gender &
        % PETA 
        69.24 &
        % RAP
        95.90 & 
        % PA-100K
        72.93 \\
        
        \hline
        \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%% PA100k %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % Modelo
        \multirow{10}{*}{PA-100K} &
        StrongBase &
        % PETA 
        77.28  &
        % RAP
        86.93 &
        % PA-100K
        \textbf{90.97} \\ 
        
        % Modelo
        &
        StrongBase-Gender &
        % PETA 
        75.01 &
        % RAP
        88.38 &
        % PA-100K
        90.77 \\
        
        
        \cline{2-5}
        
        &
        % Modelo
        ALM  &
        % PETA 
        75.48 &
        % RAP
        85.87 &
        % PA-100K
        88.34 \\
        
        &
        ALM-Gender &
        % PETA 
        76.59 &
        % RAP
        88.55 &
        % PA-100K
        90.34 \\ 
        
        \cline{2-5}
        % Modelo
        &
        DeepMar &
        % PETA 
        76.17 &
        % RAP
        85.73 &
        % PA-100K
        88.52 \\
        
        % Modelo
        &
        DeepMar-Gender &
        % PETA 
        74.50 &
        % RAP
        85.72 &
        % PA-100K
        90.39 \\

        \cline{2-5}
        % Modelo
        &
        VAC &
        % PETA 
        75.20 &
        % RAP
        87.79 &
        % PA-100K
        90.17 \\

        % Modelo
        &
        VAC-Gender &
        % PETA 
        76.85 &
        % RAP
        88.98&
        % PA-100K
        91.05 \\
        
        \cline{2-5}
        % Modelo
        &
        APR &
        % PETA 
        76.53 &
        % RAP
        87.24 &
        % PA-100K
        89.91 \\
        
        % Modelo
        &
        APR-Gender &
        % PETA 
        75.26 &
        % RAP
        86.29 &
        % PA-100K
        90.05 \\

        \hline
    \end{tabular}
    \label{table:cross_domain}
\end{table}

% \begin{table*}[!htb]
%     \renewcommand{\arraystretch}{1.2}
%     \caption{Pedestrian attribute metric values in PETA dataset.}
%     \begin{tabular}{c*{5}c|*{5}c|*{5}c}\\\hline
%         \multirow{2}{*}{\textbf{Methods}} & \multicolumn{5}{c|}{PETA}
%         & \multicolumn{5}{c|}{RAP} & \multicolumn{5}{c}{PA-100K} \\

%         &\makebox[1em]{\footnotesize mA}
%         &\makebox[1em]{\footnotesize Acc}
%         &\makebox[1em]{\footnotesize Prec}&\makebox[1em]{\footnotesize Recall}&\makebox[1em]{\footnotesize F1}
        
%         &\makebox[1em]{\footnotesize mA}
%         &\makebox[1em]{\footnotesize Acc}
%         &\makebox[1em]{\footnotesize Prec}&\makebox[1em]{\footnotesize Recall}&\makebox[1em]{\footnotesize F1}
        
%         &\makebox[1em]{\footnotesize mA}
%         &\makebox[1em]{\footnotesize Acc}
%         &\makebox[1em]{\footnotesize Prec}&\makebox[1em]{\footnotesize Recall}&\makebox[1em]{\footnotesize F1}
%         % &\makebox[4em]{\footnotesize Gender Acc}
%         \\\hline\hline

%         VAC \cite{guo2019visual} &
%         % mA 
%         82.34 & 
%         % Acc, Prec, Recall, F1
%         78.80 & \textbf{89.15} & 84.08 & 86.16 &
        
%         % mA 
%         75.11 & 
%         % Acc, Prec, Recall, F1
%         68.34 & \textbf{83.52} & 77.25 & 79.84 &
        
%         78.20 & 
%         % Acc, Prec, Recall, F1
%         \textbf{79.80} & \textbf{90.95} & 84.98 & \textbf{87.44} \\
        
%         % Modelo
%         ALM \cite{tang2019improving} &
%         % mA 
%         82.48 & 
%         % Acc, Prec, Recall, F1
%         77.25 & 85.24 & 85.61 & 85.13 & 
        
%          % mA 
%         \textbf{80.68} & 
%         % Acc, Prec, Recall, F1
%         66.73 & 73.69 & \textbf{86.19} & 78.99 &
        
%         % mA 
%         78.75 & 
%         % Acc, Prec, Recall, F1
%         75.80 & 82.94 & \textbf{87.78} & 84.79 \\
        
%         % Modelo
%         APR \cite{lin2019improving} &
%         % mA 
%         82.83 & 
%         % Acc, Prec, Recall, F1
%         77.90 & 86.99 & 84.69 & 85.52 &
        
%         % mA 
%         73.44 & 
%         % Acc, Prec, Recall, F1
%         67.12 & 82.39 & 76.33 & 78.85 &
        
%         % mA 
%         77.33 & 
%         % Acc, Prec, Recall, F1
%         78.00 & 88.34 & 85.08 & 86.24\\
        
%         % Modelo
%         DeepMar \cite{li2015multi} &
%         % mA 
%         83.89 & 
%         % Acc, Prec, Recall, F1
%         76.81 & 85.16 & 84.81 & 84.98 &
        
%         % mA 
%         77.06 & 
%         % Acc, Prec, Recall, F1
%         64.05 & 76.46 & 77.96 & 76.70 & 
        
%         % mA 
%         79.26 & 
%         % Acc, Prec, Recall, F1
%         76.48 & 85.49 & 85.71 & 85.15 \\

%         % Modelo
%         StrongBase \cite{jia2020rethinking} &
%         % mA 
%         \textbf{85.30} & 
%         % Acc, Prec, Recall, F1
%         \textbf{79.00} & 86.62 & \textbf{86.52} & \textbf{86.30} &
        
%         % mA 
%         80.61 & 
%         % Acc, Prec, Recall, F1
%         \textbf{68.63} & 79.86 & 81.13 & \textbf{80.10} & 
        
%         % mA 
%         \textbf{80.55} & 
%         % Acc, Prec, Recall, F1
%         79.06 & 87.51 & 87.13 & 86.93 \\
    

%         \hline
%     \label{table:reported_results}
%     \end{tabular}
% \end{table*}


From this experiment, we can observe that gender training models have slightly better gender accuracy when compared to all attribute trained models. This effect is present in scenarios where the model was trained and evaluated in the same dataset and when the model is trained and evaluated in different datasets. As such, in the remaining experiments, we will use gender-trained models.

Regarding gender accuracy across models, we can conclude that no model is significantly better than the others in gender prediction, regardless of the dataset where it was trained or evaluated. However, examining models' performances within and across datasets suggests dataset differences linked to gender prediction accuracy. First, models trained in PETA or PA-100K and evaluated in other datasets tend to perform well, achieving results close to those they present when evaluated in the same dataset they were trained. Second, considering same dataset train and evaluation, RAP is the dataset where models perform the best, achieving the highest gender accuracy out of all the three evaluated datasets. Finally, models trained in RAP perform considerably worse in other datasets, and models trained in PETA or PA-100K achieve better performances in RAP than in any other dataset, aside from the one they were trained in. These observations indicate that the RAP dataset images may contain features that are easier for models to predict gender and that PETA is the most challenging dataset, of the selected three, for gender prediction. % PETA conclusion is right but not explained...


\subsection{Dataset Analysis}
% Presentation of image aspect for each dataset plus dataset of only frontal images. The main conclusion is that PETA is a lower quality dataset with smaller and blurrier images, while RAP is a higher quality dataset with higher resolution images and significantly less blurrier images. PA100k is of intermediate quality in terms of resoltuion and blurriness. Luminosity is constant across all three datasets. Frontal substets of each dataset present the same characteristics of the full dataset.

To understand how image features influence gender prediction, we evaluate them on the three pedestrian attribute datasets. We normalize the values obtained for each feature and represent the mean and standard deviation of each, for all datasets, in Table \ref{table:dataset_analysis}. 

\begin{table}[!t]
    \renewcommand{\arraystretch}{1.1}
    \centering
    \caption{Dataset attributes.}
    \begin{tabular}{|c|*{3}{c|}}\hline
        \textbf{Dataset}  & 
        \textbf{Resolution} &
        \textbf{Luminosity} &
        \textbf{Blurriness} 
        \\\hline\hline
        
        PETA &
        0.037 $\pm$ 0.024 &
        0.432 $\pm$ 0.100 &
        0.120 $\pm$ 0.148 \\

        RAP & 
        0.131 $\pm$  0.083 &
        0.407 $\pm$  0.107 & 
        0.022 $\pm$  0.013 \\
        
        PA-100K & 
        0.062 $\pm$ 0.063 &
        0.449 $\pm$ 0.126 & 
        0.095 $\pm$ 0.089 \\

        
        % PETA &
        % 13295.176 $\pm$ 8058.963 &
        % 110.986 $\pm$ 23.921 &
        % 1755.199 $\pm$ 2132.994 \\
 
        % RAP & 
        % 45436.862 $\pm$  28026.175 &
        % 105.464 $\pm$  25.381 & 
        % 327.092 $\pm$  191.258 \\
        
        % PA100k & 
        % 18822.201 $\pm$ 17803.808 &
        % 105.543 $\pm$ 29.856 & 
        % 1248.960 $\pm$ 1336.077 \\
        \hline
        
    \end{tabular}
    \label{table:dataset_analysis}
\end{table}


Given the non-variation of luminosity across the datasets, we group datasets into quality categories based on resolution and blurriness: low, medium, and high. The higher quality dataset is RAP, given the high resolution value and a low one of blurriness. PETA is the dataset with lower quality, based on the low resolution values and high values (with high variance) of blurriness. Since PA-100K dataset feature values are between those of PETA and RAP, we consider this dataset as of medium quality. We represent a quality bar of the three evaluated datasets in Figure \ref{fig:gradient_quality}, accompanied by image examples of each dataset.

In conjunction with cross-domain performance results, this analysis suggests that higher gender prediction accuracy might be linked to higher quality images and lower accuracy to poorer quality images.

\begin{figure}[!htb]
\centering
\includegraphics[scale=0.55]{imgs/gradient_quality.pdf}
\caption{Simulation results for the network.}
\label{fig:gradient_quality}
\end{figure}



\subsection{Methods Prediction Evaluation}
% Presentation of table with image and person aspects. The results presented consider all the methods by considering correct image as an image where are least one of the selected methods failed. This approach is admissible given the high value of all methods for gender prediction. From this analysis, overall, images where a person is back tend to be where a method fails less and sideways is where methods fail more. This effect is more visible in PETA, where images are of lower quality. Conclusion: there are other image aspects aside from person orientation that might influence prediction. Look at them in next section


We evaluated the correctly gender-predicted image features and compared them to all test set dataset image features to understand what characteristics contribute the most to gender misprediction. This experiment evaluates image and person-related features, namely
orientation and keypoint (KP) confidence. We only evaluated misprediction from models when trained and evaluated in the same dataset. Additionally, given all models' high accuracy, we grouped their predictions and considered images as correctly gender-predicted when all models correctly predicted the gender. We present our results in Table \ref{tabel:method_prediction}; all values displayed are normalized to each dataset.

\begin{table*}[!t]
    \centering
    \caption{Gender prediction images feature for all five evaluated methods, for PETA, RAP and PA100k datasets. The images considered as corrected are those where all methods correctly predict the gender. \texttt{Correct} refers to correctly predicted images and \texttt{All} refers to all dataset test images.}
    \begin{tabular}{|cl||*{6}{c|}}\hline
        % \backslashbox{\textbf{Features}}{\textbf{Model}}  & PETA & 
        % PETA Gender & RAP & RAP Gender & PA100k & PA100k Gender &
        % \textbf{Dataset}
        % \\\hline\hline
        
        \multicolumn{2}{|c||}{\multirow{2}{*}{\textbf{Features}}} & \multicolumn{2}{c|}{PETA}  &
        \multicolumn{2}{c|}{RAP} & \multicolumn{2}{c|}{PA100k} \\
        & & Correct & All  & Correct & All & Correct & All
        \\\hline\hline
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%% Person Orientation %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \multirow{3}{*}{Person Orientation}  
                        % PETA   
        & Front         & 0.38 & 0.38 
                        % RAP
                        & 0.35 & 0.35 
                        % PA100k
                        & 0.36  & 0.36   \\
        
                        % PETA   
        & Back          & 0.39 & 0.37  
                        % RAP
                        & 0.34 & 0.34 
                        % PA100k
                        & 0.28  & 0.28   \\
        
                        % PETA   
        & Sideways      & 0.22 & 0.25  
                        % RAP
                        & 0.31 & 0.32 
                        % PA100k
                        & 0.36  & 0.37   \\
         \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%% KP Probability %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \multirow{3}{*}{KP Confidence}
                      % PETA   
        & Face          & 0.82 $\pm$  0.11 & 0.82 $\pm$  0.11 
                        % RAP
                        & 0.84 $\pm$  0.12 & 0.84 $\pm$  0.13
                        % PA100k
                        & 0.82 $\pm$  0.12  & 0.81 $\pm$  0.13   \\
        
                        % PETA   
        & Upper Body    & 0.78 $\pm$  0.11 & 0.78 $\pm$  0.11  
                        % RAP
                        & 0.82 $\pm$  0.10 & 0.82 $\pm$  0.10
                        % PA100k
                        & 0.77 $\pm$  0.10  & 0.77 $\pm$  0.10   \\
        
                        % PETA   
        & Lower Body    & 0.76 $\pm$  0.11 & 0.76 $\pm$  0.11  
                        % RAP
                        & 0.79 $\pm$  0.12 & 0.78 $\pm$  0.12  
                        % PA100k
                        & 0.77 $\pm$  0.09 & 0.76 $\pm$  0.09     \\
        
        \hline
        %%%%%%%%%%%%%%%%%%%%%%%%%%% Image %%%%%%%%%%%%%%%%%%%%%%%%%%%%      
        \multirow{3}{*}{Image} 
                        % PETA   
        & Resolution    & 0.21 $\pm$  0.13 & 0.21 $\pm$  0.13
                        % RAP
                        & 0.22 $\pm$  0.16 & 0.23 $\pm$  0.16 
                        % PA100k
                        & 0.07 $\pm$  0.12  & 0.06 $\pm$  0.07  \\
        
                        % PETA   
        & Luminosity    & 0.42 $\pm$  0.12 & 0.42 $\pm$  0.12
                        % RAP
                        & 0.45 $\pm$  0.16 & 0.46 $\pm$  0.16 
                        % PA100k
                        & 0.48 $\pm$  0.15  & 0.48 $\pm$  0.15   \\
        
                        % PETA   
        & Blurriness    & 0.15 $\pm$  0.19 & 0.14 $\pm$  0.18 
                        % RAP
                        & 0.12 $\pm$  0.07 & 0.11 $\pm$  0.07  
                        % PA100k
                        & 0.11 $\pm$  0.12 & 0.11 $\pm$  0.12     \\

        \hline
    \end{tabular}
    \label{tabel:method_prediction}
\end{table*}


The results suggest no significant differences between images where gender was correctly predicted and all test set images for all evaluated features. The only case where we found a more significant difference was in PETA, where models had better performance in images where the person was not facing forward (\textit{Back}) and a worse one where the person was facing sideways. To confirm that the orientation was the factor influencing gender prediction, we analyzed image-related features and KP confidence of all sideways and back images of PETA. The obtained results are exhibited in Table \ref{table:PETA_side_back}.

\begin{table}[!t]
    \centering
    \caption{Analysis of back and sideways images features compared to all images of PETA. \texttt{Back} refers to back images, \texttt{Sideways} to side images and \texttt{All} refers to all dataset test images.}
    \begin{tabular}{|cl|*{3}{c|}}\hline

        \multicolumn{2}{|c|}{\multirow{2}{*}{\textbf{Features}}} & \multicolumn{3}{c|}{PETA} \\
        & & Back & Sideways & All
        \\\hline\hline
      %%%%%%%%%%%%%%%%%%%%%%%%%%% KP Probability %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \multirow{3}{*}{KP}
                      % PETA   
        & Face          & 0.76 $\pm$  0.08 & 
                        0.81 $\pm$  0.11 & 
                        0.82 $\pm$  0.11  \\
    
                        % PETA   
        & Upper Body    & 0.78 $\pm$  0.09 & 
                        0.70 $\pm$  0.13 & 
                        0.78 $\pm$  0.11  \\
        
                        % PETA   
        & Lower Body    & 0.77 $\pm$  0.10 & 
                        0.71 $\pm$  0.13 & 
                        0.76 $\pm$  0.11   \\
        
        \hline

        %%%%%%%%%%%%%%%%%%%%%%%%%%% Image %%%%%%%%%%%%%%%%%%%%%%%%%%%%    
        \multirow{3}{*}{Image} &
                        % PETA   
        Resolution    & 0.22 $\pm$  0.14 & 
                        0.16 $\pm$  0.11 & 
                        0.21 $\pm$  0.13 \\
        
                        % PETA   
        & Luminosity    & 0.44 $\pm$  0.12 & 
                        0.41 $\pm$  0.12 & 
                        0.42 $\pm$  0.12  \\
        
                        % PETA   
        & Blurriness    & 0.11 $\pm$  0.15 & 
                        0.11 $\pm$  0.14 &
                        0.14 $\pm$  0.18  \\
        \hline
    \end{tabular}
    \label{table:PETA_side_back}
\end{table}

Based on the results, person orientation might not be the contributing factor for gender prediction accuracy. In the PETA dataset, images where the person is not facing forward are higher quality images, translated by higher resolution, luminosity, and lower blurriness, than all test set images. An analogous analysis can be made for sideways images where these are considered lower quality than the average of test set images. Additionally, this type of image is linked to lower confidence of the upper and lower body, which is admissible given the lower percentage of visible body in images where a person is facing sideways. This fact can also justify, in addition to the image quality, a lower gender prediction accuracy in this type of image.

This experiment clarified that a general feature evaluation of correctly gender-predicted images might not be enough to identify how each feature contributes to gender prediction accuracy. 

\subsection{Interpreting Gender Prediction}
\label{sec:shap_results}

% For a granular aspect evaluation, we gather each image information and grouped it with the correspondent output of 0 if said image was mispredicted and 1 otherwise. After, we gave it to a SHAP model (??) and analyzed which features contributed the most for model output. We gathered person orientation into a single attribute, orientation, wher 0 is frontal, 0.5 sideways and 1 back. 

% First, we grouped all dataset to evaluate image aspect influence in gender prediction. From this analyzis we can see that ...

% To understand when some image aspects might be more important we performed the same analysis for each dataset. For PETA, representing lower quality images, non person related aspects acquire more importance. Furthermore, blurriness appears to have an importance in these images, which does not translate into higher quality images. From pa100k to rap, face and lower body gain importance. Given an higher resolution image, the KP confidence rises which promotes an importance elevation for gender prediction. While in lower images face influence may be lower, here it gains relevance. In images with high quality and low blurriness, such as RAP, the considered aspects have little impact in gender prediction. This suggest that this is a threshold where increase of resolution does not translate in better model performance. 

With the intent to interpret feature values of different quality images and their correlation with gender prediction, we grouped all the model predictions for all datasets. We obtain feature values of each test sets image for all datasets and associated a value 1 to it if all models correctly predicted the gender and 0 otherwise. Finally, we process this information using the framework SHAP (SHapley Additive exPlanations) \cite{lundberg2017unified}, a game-theoretic approach to explain any machine learning model's output, using the TreeExplainer model \cite{lundberg2020local}, from a publicly available implementation \cite{git_shap}.

Analyzing the bar plot for each feature's absolute mean values in figure 1 leads us to conclude that image resolution and lower body KP confidence are the most influential characteristics for gender prediction in wild conditions. Bars in blue are positively correlated values, while in red are negatively correlated. In this case, high values of blurriness, translated into blurrier images, contribute to gender misprediction. The resolution importance is understandable given that it is hard to differentiate gender in small pictures, and it is easier when images are bigger. The lower body importance might be related to hip or footwear influence in gender discrimination. It is admissible to consider such scenarios given that we evaluate wild conditions, with people in different poses and images with variable quality. In these cases, the person's face difficult detection and partially occluded body might contribute models to focus on other aspects for gender determination.

\begin{figure}[!htb]
\centering
\includegraphics[width=3in]{imgs/combined/general_.png}
\caption{Simulation results for the network.}
\label{fig_sim}
\end{figure}

% ALL bar plot

To better understand each feature value's correlation in gender prediction, we evaluate dependence plots for some features. Figure \ref{shap_all} presents the results for the face, lower, and upper body KP confidence, resolution, blurriness, and luminosity dependence plots; image-related features are normalized. Negative SHAP values are linked to gender misprediction, while positive ones are linked to correctly predicted gender. We can conclude that higher KP confidence values translate into gender-correct predictions. For lower and upper body KP, confidence above 0.7 is linked to correct predictions, while face KP requires the confidence of 0.8 for the same effect. Low values of resolution heavily negatively impact gender prediction and are positively influential in higher values. Luminosity only influences gender prediction when it has low values and tends to have a neutral role in higher values. Blurriness has a positive influence on low values and a negative influence when its values arise. An increase in blurriness does not translate into more incorrect gender prediction.

% ALL dependence plots
\begin{figure*}[!ht]
\centering

\subfloat[]{\includegraphics[width=2.2in]{imgs/combined/face_lower_body.png}}
\quad
\subfloat[]{\includegraphics[width=2.2in]{imgs/combined/lower_body_luminosity.png}}
\quad
\subfloat[]{\includegraphics[width=2.2in]{imgs/combined/upper_body.png}}

\subfloat[]{\includegraphics[width=2.2in]{imgs/combined/resolution.png}}
\quad
\subfloat[]{\includegraphics[width=2.2in]{imgs/combined/luminosity.png}}
\quad
\subfloat[]{\includegraphics[width=2.2in]{imgs/combined/blurriness.png}}

\caption{Simulation results for the network.}
\label{shap_all}
\end{figure*}

These results suggests that higher resolution images with good illumination, low blurriness, and cooperative people's pose (translated in high KP confidence values) are crucial elements for correct gender prediction. Another conclusion is that face might not be as reliable for wild gender prediction since it requires higher confidence values (than those of lower and upper body) for correct gender predictions.

Although an overall view of feature influence in gender prediction in wild conditions is necessary, we further investigate if image quality alters feature importance. For this, we analyze feature influence in PETA, representing lower quality images, and in RAP, containing images of high quality. 

The bar plot results for each feature's absolute mean values in PETA, exhibited in Figure \ref{shap_peta}, demonstrate the importance of image-related features for gender prediction. This analysis suggests that person-related features are not reliable for gender prediction in scenarios where image quality is subpar. The dependence plots of the image-related features corroborate the conclusion withdrawn from the overall image analysis. In situations where blurriness is high, illumination tends to improve gender prediction, as displayed in the dependence plot of blurriness per luminosity values.

% PETA bar + dependence
% \begin{figure*}[!t]
% \centering

% \subfloat[]{\includegraphics[width=2.2in]{imgs/peta/general_.png}}
% \quad
% \subfloat[]{\includegraphics[width=2.2in]{imgs/peta/blurriness_lumino.png}}
% \quad
% \subfloat[]{\includegraphics[width=2.2in]{imgs/peta/luminosity.png}}

% %\subfloat[]{\includegraphics[width=2.2in]{imgs/peta/resolution.png}}

% \caption{Simulation results for the network.}
% \label{shap_peta}
% \end{figure*}

\begin{figure}[!htb]
\centering

\includegraphics[width=2.5in]{imgs/fig.png}

\caption{Simulation results for the network.}
\label{shap_peta}
\end{figure}

% \begin{figure}[!htb]
% \centering

% \includegraphics[width=2.2in]{imgs/peta/general_.png}

% \caption{Simulation results for the network.}
% \label{shap_peta}
% \end{figure}

In Figure \ref{shap_rap}, we evaluate the bar plot of high-quality image features. The absolute values are lower than those in PETA, which indicates that gender prediction is less reliant on the evaluated features in high-quality images. In particular, face and lower body gain importance in these scenarios while blurriness and luminosity lose some. If we analyze dependence plots, we retrieve more critical information. Up to 0.6 face KP confidence, gender prediction is positively linear to KP confidence, while above this value, gender prediction correctness is not influenced. For resolution, we can observe that an increase in its value does not translate in higher gender correct predictions; only below a threshold does it negatively influence gender inference. These results suggest that, for high-quality images, an increase of resolution does not translate in higher gender prediction accuracy, and face confidence needs to be above 0.6 not to influence gender inference negatively.

% RAP bar + dependence
% \begin{figure*}[!htb]
% \centering

% \subfloat[]{\includegraphics[width=2.2in]{imgs/rap/general_.png}}
% \quad
% \subfloat[]{\includegraphics[width=2.2in]{imgs/rap/face_resolution.png}}
% \quad
% \subfloat[]{\includegraphics[width=2.2in]{imgs/rap/resolution.png}}

% \caption{Simulation results for the network.}
% \label{shap_rap}
% \end{figure*}

% \begin{figure}[!htb]
% \centering

% \includegraphics[width=2.2in]{imgs/rap/general_.png}

% \caption{Simulation results for the network.}
% \label{shap_peta}
% \end{figure}


Analyzing PA-100K images, which we considered as medium quality given its image-related feature values, allows us to observe the increase in the importance of person-related features, in particular face KP confidence. 

% PA100k bar
% \begin{figure}[!htb]
% \centering
% \includegraphics[width=2.5in]{imgs/pa100k/general_.png}
% \caption{Simulation results for the network.}
% \label{fig_sim}
% \end{figure}

Summing all the obtained results, they suggest that person-related features are not reliable in small and blurry images (low quality) and that an increase in image quality (medium quality) translates into higher person-related feature importance for gender prediction. If the images are high-quality (high resolution and low blurriness), image and person-features lose importance since an increase in its values does not translate into better model performance.


\subsection{Face Importance in Gender Prediction}

% Firstly, we intent to analyze face gender model, trained in Adience, and evaluated in wild image conditions. It is important to note that, while in Adience the images and orientation and the person is facing the camera, such considerations are absent in wild conditions. This analysis is meant to evaluate the applicability of models trained in face datasets in wild scenarios. To keep it as fairly as possible, we extracted face images from frontal images of each dataset. As observed, the perfomance is subpar, when compared to the 94\% obtained in one of the most challenging face datasets. Cross evaluation was also performed in models trained for different frontal datasets.

% SHAP analysis for face? Model trained for face images of all 3 datasets

% SHAP hints that face importance might be linked to higher quality images. To corroborate such idea we trained face gender model in all images of dataset and in only frontal images of dataset. Then, we evaluted each of the two models in only face images of each dataset. The results in table X suggest that the model trained in RAP are able to more accurately predict gender based solely on face images, which suggest that face has higher importance in images with higher resolution. Additionally, forcing the model to train solely on frontal images, increases face importance for gender prediction. The importance of face is translate in a percentage number, where the min admissible is 50\% (random) and the max is the value obtained for body image evaluation.

The results obtained in section \ref{sec:shap_results} suggest that face importance for gender prediction might be related to image quality increase. To explore this topic, we use our face gender model and train it on Adience, one of the most challenging face gender datasets. We present the gender accuracy obtained for our model in Table \ref{table:adience}, comparing it with reported results.

% Table Adience
\begin{table}[!htb]
    \centering
    \caption{Gender accuracy of ResNet50 model trained and evaluated in different face datastes. PETA, RAP and PA100k datasets were adapted to contain only faces of frontal people images.}
    \begin{tabular}{|c||*{9}{c|}}\hline
        \backslashbox{\textbf{Train}}{\textbf{Eval}} & \multicolumn{1}{c|}{Adience}
        % & \multicolumn{2}{c|}{PETA} 
        & \multicolumn{1}{c|}{PETA Face} 
        & \multicolumn{1}{c|}{RAP Face} 
        & \multicolumn{1}{c|}{PA100k Face} 
        \\\hline\hline
        % \textbf{Metrics} &
        % \makebox[1em]{Acc} &
        % % \makebox[1em]{Acc}&\makebox[1em]{mA} &
        % \makebox[1em]{Acc} &
        % \makebox[1em]{Acc} &
        % \makebox[1em]{Acc}
        % \\\hline\hline
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%% Adience Model %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        Adience &
        
        % Adience
        % Acc, mA, 
         94.83 &
        
        % % PETA
        % % Acc, mA, 
        % 55.04 & 58.40 &
        
        % PETA Frontal
        % Acc, mA,
        65.56 &
        
        % RAP Frontal
        % Acc, mA,
        77.85 & 
        
        % PA100k Frontal
        % Acc, mA,
        55.55 \\
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%% PETA Frontal Model %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        PETA Face &
        
        % Adience
        % Acc, mA, 
        64.96 &
        
        % % PETA
        % % Acc, mA, 
        % 79.74 & 79.81 &
        
        % PETA Frontal
        % Acc, mA,
         91.16 &
        
        % RAP Frontal
        % Acc, mA,
        82.43 &
        
        % PA100k Frontal
        % Acc, mA,
        74.60 \\
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%% RAP Frontal Model %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        RAP Face &
        
        % Adience
        % Acc, mA, 
        75.49 &
        
        % % PETA
        % % Acc, mA, 
        % - & - &
        
        % PETA Frontal
        % Acc, mA,
        68.09 &
        
        % RAP Frontal
        % Acc, mA,
         95.31 &
        
        % PA100k Frontal
        % Acc, mA,
        68.32 \\
        
        %%%%%%%%%%%%%%%%%%%%%%%%%%% PA100k Frontal Model %%%%%%%%%%%%%%%%%%%%%%%%%%%%
        PA100k Face &
        
        % Adience
        % Acc, mA, 
        75.62 &
        
        % % PETA
        % % Acc, mA, 
        % - & - &
        
        % PETA Frontal
        % Acc, mA,
        72.52  &
        
        % RAP Frontal
        % Acc, mA,
        79.72  &
        
        % PA100k Frontal
        % Acc, mA,
         84.71 \\
        
        \hline
    \end{tabular}
    \label{table:adience}
\end{table}

The obtained accuracy is better than the reported ones, indicating that our model represents a good face gender model. To analyze the applicability of face gender trained models in detecting gender in wild conditions, we promoted a cross-domain performance in models using Adience, PETA, RAP, and PA-100K datasets for training and evaluation. To keep the Adience analysis comparison as fair as possible, we trained and evaluated models in PETA, RAP, and PA-100K using only face images of frontal people of each dataset. We report our results in Table \ref{table:face_imp}.

% Table face cross evaluation
\begin{table*}[!htb]
    \centering
    \caption{Gender accuracy of ResNet50 model trained for any orientation body images and evaluated in frontal face and any orientation body images, of various pedestrian datasets. Face importance is calculated based on mA. Face evaluation refers to frontal image face extracted images evaluation. \texttt{Face Imp} stands for Face Importance. }
    \begin{tabular}{|c||*{6}{c|}}\hline
        \multicolumn{1}{|c||}{\textbf{Trained}} & \multicolumn{3}{c|}{\textbf{Any Orientation Body}} & \multicolumn{3}{c|}{\textbf{Frontal Body}}  \\\hline\hline
        \backslashbox{\textbf{Dataset}}{\textbf{Evaluated}} & 
        \multicolumn{1}{c|}{Face} & 
        \multicolumn{1}{c|}{Body} &
        \multicolumn{1}{c|}{Face Imp} &
        \multicolumn{1}{c|}{Face} & 
        \multicolumn{1}{c|}{Body} &
        \multicolumn{1}{c|}{Face Imp}\\\hline\hline
        \textbf{Metrics} &
        \makebox[1em]{mA} &
        \makebox[1em]{mA} &
        \makebox[1em]{\%} &
        \makebox[1em]{mA} &
        \makebox[1em]{mA} &
        \makebox[1em]{\%} \\
        \hline\hline
        PETA & 
        57.60 & 92.88 & 17.72 &
        55.89 & 92.63 & 13.82 \\
        
        RAP & 
        73.63 & 96.09 & 51.27 &
        75.31 & 95.98 & 55.05 \\
        
        PA100k &
        52.52 & 91.06 & 6.14 &
        61.46 & 91.24 & 27.79 \\
        
        % RAP+PA100k & 63.73 & 56.91 & 70.64 & 71.30 & 32.44 \\
        \hline
    \end{tabular}
    \label{table:face_imp}
\end{table*}

We can observe that Adience trained model performs poorly in other datasets, illustrating that face gender training is not adequate for wild gender inference. However, the dataset where this model performed the best was RAP, characterized as a high-quality image dataset. Similarly, RAP-trained models achieve higher accuracy performance in Adience than in PETA or PA-100K. These results indicate that Adience and RAP-Frontal are similar datasets which might indicate that face importance is closely related to increased image quality.

To further explore this concept, we trained our face gender model in all dataset images (whole-body) and evaluated its gender prediction performance when evaluated in face images of the same dataset. Furthermore, we performed the same procedure but training the model only in frontal dataset images. We present the obtained results in Table 6.

% Table all vs frontal in face importance

The results suggest that, when training for the whole body and given face images for gender inference, models trained in RAP have significantly better performance than those of PETA or PA-100K. This analysis suggests that higher quality images influence face importance in gender prediction. Furthermore, when we train the model with frontal images only and evaluated gender prediction using face images, the face importance increases for all three datasets. This result suggests that face importance is also linked to its availability which is not a guaranteed condition in wild conditions. However, if we guarantee face availability by training the model in frontal images only, the model can attribute higher face significance, translating in better performances when evaluated in face images.

% Referir importância de cognição para este resultado? Novas vias a explorar?

To evaluate that person orientation was the factor contributing to increased face importance, we analyzed image-related features in frontal images for each dataset. The results of Table \ref{table:frontal_all} demonstrate that frontal images have a similar quality to all test set dataset images, which confirms that person orientation was the driving factor for increased face importance.
% Table all vs frontal = same characteristics


% \begin{table}[!htb]
%     \centering
%     \caption{Dataset attributes normalized. Frontal datasets attribute values presented are related to full body images.}
%     \begin{tabular}{|c||*{5}{c|}}\hline
%         \textbf{Dataset} & 
%         Resolution &
%         Luminosity &
%         Blurriness 
%         \\\hline\hline
        
%         PETA &
%         0.037 $\pm$ 0.024 &
%         0.432 $\pm$ 0.100 &
%         0.120 $\pm$ 0.148 \\
        
%         PETA-Frontal &
%         0.037 $\pm$ 0.023 &
%         0.437 $\pm$ 0.101 &
%         0.140 $\pm$ 0.158 \\

%         \hline
%         RAP & 
%         0.131 $\pm$  0.083 &
%         0.407 $\pm$  0.107 & 
%         0.022 $\pm$  0.013 \\
        
%         RAP-Frontal & 
%         0.138 $\pm$  0.090 &
%         0.416 $\pm$  0.108 & 
%         0.023 $\pm$  0.013 \\
        
%         \hline
%         PA-100K & 
%         0.062 $\pm$ 0.063 &
%         0.449 $\pm$ 0.126 & 
%         0.095 $\pm$ 0.089 \\

%         PA-100K-Frontal & 
%         0.061 $\pm$ 0.064 &
%         0.459 $\pm$ 0.127 & 
%         0.100 $\pm$ 0.090 \\
%         \hline
        
%     \end{tabular}
%     \label{table:frontal_all}
% \end{table}

% Referir importância de cognição para este resultado? Novas vias a explorar?

==> article/intro_prev.tex <==

\section{Introduction}
% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by the IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.
% \IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
% for IEEE journal papers produced under \LaTeX\ using
% IEEEtran.cls version 1.8b and later.

\begin{figure*}[!htb]
\centering
\includegraphics[width=7in]{imgs/main_image.pdf}
\caption{Overview of used approaches for image and person-based features in gender prediction and the importance of face for such a task in wild conditions. We divide the approaches into three major steps: Image Quality Division, Gender Inference Interpretation, and Face Importance Analysis. We divide PAR datasets based on the image-based feature values of their images. Then, we analyze datasets images based on image and person-based features and image quality, correlating them with a meta model gender prediction. Meta gender model is a combination of five different PAR models. Face importance is analyzed in two ways: evaluating its reliability and assessing orientation influence in wild face image gender prediction. Face reliability for gender prediction is analyzed by training a proposed face gender model in Adience, a face gender dataset, and evaluating its performance in wild face images. Orientation influence in face importance is examined by training the proposed face gender model in frontal or all dataset images and evaluating their gender prediction accuracy when given face images.
}
\label{fig:main_image}
\end{figure*}

% This work was developed in the context of Human Behavior Analysis, which has been gaining increasing interest over the last years, given its importance in societal needs such as security, affective computing, assisted living, and abnormal situation detection \cite{yu2020human}. This interest is also enhanced by the availability of massive amounts of data in \emph{wild} conditions, provided by surveillance cameras and footage gathered by hand-held devices. In particular, it is known that soft biometric features can play an important role in the behavior of individuals among crowds. 

Soft Biometrics Analysis has been gaining increasing interest over the last years, given its importance in societal needs such as security, affective computing, assisted living, and abnormal situation detection \cite{yu2020human}. This interest is also enhanced by the availability of massive amounts of data in \emph{wild} conditions, provided by surveillance cameras and footage gathered by hand-held devices. In this context, soft biometric features can play an important role in the behavior of individuals among crowds. 

% Even though the soft biometrics inference is frequently seen as a relatively easy (solved) task, this work reports the results observed in extensive analysis that points for the opposite. In particular, we have posed the following research questions:

Even though soft biometrics inference is frequently seen as a relatively easy (solved) task, this work reports the results observed from an extensive analysis that points to the opposite. In particular, we pose the following research questions:

\begin{itemize}
    \item \textbf{How well solved is wild soft biometric estimation?}
    \item  \textbf{What features have the most relevance for soft biometrics inference accuracy?}
    % \item \textbf{Given the face importance in some of the soft biometrics described, what conditions can justify its use in wild soft biometrics prediction?}
    \item \textbf{Given the face importance in some existing soft biometrics, what conditions can justify its use in wild soft biometrics prediction?}
\end{itemize}

% To provide answers to the above questions, we focused in particular the \emph{gender} trait, which can be retrieved from an image and is influenced by the human silhouette and face. However, the conclusions yielding from such analysis may apply to other soft biometrics traits, such as ``age'', ``body mass'', or ``ethnicity''.

To provide answers to the above questions, we focus, in particular, on the \emph{gender} trait, which can be retrieved from an image and is influenced by the human silhouette and face. However, the conclusions yielding from such analysis may apply to other soft biometrics traits, such as \emph{age}, \emph{body mass}, or \emph{ethnicity}.

The gender as a discriminative behavioral feature has been the topic of many psychology studies. The choice of clothes, interests, and friendships are associate with gender expression and differentiate women and men \cite{gender_exp}. Regarding exploration, women present a more calculated approach to explore, which results in increased pausing behaviors \cite{exploration_gender}. In the context of physical human interaction, men respond less positively to touch when compared with women \cite{touch_men_women}, while women tend to be more empathic than men \cite{gender_empathy} and more reactive to unpleasant events \cite{gender_unplesant}. In social interactions, namely with comfortable interpersonal distance, height was positively associated with said distance for men but not for women \cite{height_men_women}. This set of differences between genders illustrates different behavioral responses to the same scenario, suggesting that gender is a contributing factor in human behavior analysis.

Gender prediction in wild conditions, such as surveillance environments, contains numerous challenges that affect deep learning model performance: occlusion, non-cooperative people's pose, camera quality, weather conditions, people's distance to the camera. In sum, people's pose and image quality are two key factors that influence gender prediction in wild scenarios. To achieve a reliable gender inference in this context, we need to correlate image features' importance to models' gender prediction accuracy and evaluate if said features' importance varies depending on the image quality. To achieve this goal, we define quantifiable image and person-based features and use said features to categorize image quality. We define resolution, luminosity, and blurriness as influential image-based features and face, upper and lower body keypoints (KP) confidence as person-based features. We made use of pose estimation to aid us in person-related features.

Given the intent to evaluate gender in wild conditions, we use the most variable and state-of-the-art pedestrian attribute datasets. Furthermore, to obtain a generic deep learning model performance evaluation, we gathered five state-of-the-art pedestrian attribute models and combined their predictions to obtain model-independent gender inference. To understand each considered feature's importance, we correlate them with models' combined gender prediction and analyze it using Shapley values \cite{shapley1953value}, a game-theoretic approach to explain machine learning model's output.

One other important component to analyze, regarding features' influence in wild gender prediction, is the face reliability for this task. Given that the face is one of the most defining attributes of gender distinction, several models and datasets have been created using only the face for gender inference. However, face usage in wild situations is not a guaranteed condition, and its usage requires the meeting of specific aspects. To explore this concept, we compare a model's performance trained in Adience, a face gender dataset, and evaluate it in wild face gender datasets. We construct such datasets by extracting faces from frontal images of PAR datasets, using pose estimation to aid us in this task. 

Gender detection using face may not be favored in varying scenarios of surveillance context, such as when the person is facing back or when the image resolution is too small. As such, we intend to analyze which wild conditions are adequate for face-based gender inference and investigate if it is possible to promote an increase in face importance in such a task. This logic is linked to the human cognitive capacity of preceding face prediction with person orientation: if the person faces forward, we tend to analyze the face; otherwise, we look for other clues such as person hair or silhouette. This objective was achieved by training a model in full-body datasets and evaluate its performance in face datasets. We divided face datasets based on image quality to relate it with face importance.

The main contributions of this work can be summarized as follows:
\begin{itemize}
    \item We define the most relevant image and person-based features for gender prediction and relate their importance with image quality;
    \item We present image conditions where the face can aid gender prediction in wild conditions and exhibit the pose orientation influence in face importance in such scenarios;
    \item We present a wild face image dataset creation by face extraction of frontal Pedestrian Attribute Recognition (PAR) dataset images, using a pose estimation method to aid in such a task.
\end{itemize}

The remainder of this paper is organized as follows: Section \ref{sec:gender-estimation} summarizes the most relevant face and body-based methods in gender inference; Section \ref{sec:methodology} describes the methodologies used for feature analysis, gender prediction accuracy correlation with analyzed features, and the applicability of pose estimation for head extraction; Section \ref{sec:experiments} discusses the results obtained in our experiments of feature correlation with gender prediction accuracy, and face importance relation with image quality and person orientation; main conclusions and future work are presented in Section \ref{sec:conclusion}.

